Distinct Sampling on Streaming Data with Near-Duplicates

In this paper we study how to perform distinct sampling in the streaming model where data contain near-duplicates. The goal of distinct sampling is to return a distinct element uniformly at random from the universe of elements, given that all the near-duplicates are treated as the same element. We also extend the result to the sliding window cases in which we are only interested in the most recent items. We present algorithms with provable theoretical guarantees for datasets in the Euclidean space, and also verify their effectiveness via an extensive set of experiments.

==> exp-place-holder.tex <==
\section{Experiments}

We have conducted an extensive set of experiments for our algorithm in the infinite window case.  Due to the space constraints we delay the whole section to Appendix~\ref{sec:exp}.

==> exp.tex <==
\newcommand{\randfive}{{\tt Rand5}}
\newcommand{\randfivepl}{{\tt Rand5-pl}}
\newcommand{\randtt}{{\tt Rand20}}
\newcommand{\randttpl}{{\tt Rand20-pl}}
\newcommand{\yacht}{{\tt Yacht}}
\newcommand{\yachtpl}{{\tt Yacht-pl}}
\newcommand{\seeds}{{\tt Seeds}}
\newcommand{\seedspl}{{\tt Seeds-pl}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\pTime}{\texttt{pTime}}
\newcommand{\pSpace}{\texttt{pSpace}}
\newcommand{\stdDevNm}{\texttt{stdDevNm}}
\newcommand{\maxDevNm}{\texttt{maxDevNm}}
\newcommand{\searchAdj}{\textsc{SearchAdj}}
\newcommand{\nruns}{\text{\#runs}}
\section{Experiments}
\label{sec:exp}
In this section, we present our experimental results as well as some implementation details.


\subsection{The Setup}
\paragraph{Datasets} We verify our algorithms using the following real and synthetic datasets. 
\begin{itemize}
\item \randfive: $500$ randomly generated points  in $\mathbb{R}^5$; each coordinate is a random number from $(0, 1)$.
\item \randtt: $500$ randomly generated points in $\mathbb{R}^{20}$; each coordinate is a random number from $(0, 1)$.
\item \yacht: $308$ points taken from the UCI repository yacht hydrodynamics data set.\footnote{\url{https://archive.ics.uci.edu/ml/datasets/Yacht+Hydrodynamics}} Each point is in $\mathbb{R}^7$, and it measures the sailing yachts movement.
\item \seeds:  $210$ points taken from the UCI repository seeds data set.\footnote{\url{https://archive.ics.uci.edu/ml/datasets/seeds}} Each point is in $\mathbb{R}^8$, consisting of measurements of geometrical properties of kernels belonging to three different varieties of wheat.
\end{itemize}

We perform two types of near-duplicate generations on each dataset.   In the first transformation we generate near-duplicates as follows: We first rescale the dataset such that the minimum pairwise distance is $1$. Then for each point $\bx_i\ (i = 1, 2, \ldots, n)$, we pick a number $k_i$ uniformly at random from ${1, 2, \ldots, 100}$, and add $k_i$ near-duplicate points w.r.t. $\bx_i$, each of which is generated as follows:
\begin{enumerate}
\item Generate a vector $\bz \in \mathbb{R}^d$ such that each coordinate of $\bz$ is chosen randomly from $(0,1)$.

\item Randomly sample a number $\ell \in \left(0, \frac{1}{2 d^{1.5}}\right)$ and rescale $\bz$ to length $\ell$.  Let $\hat{\bz}$ be the resulting vector.

\item Create a near-duplicate point $\by = \bx_i + \hat{\bz}$.
\end{enumerate}
Note that each point $\bx_i$, together with the near-duplicate points around it, forms a group.
We still name the resulting datasets as \randfive, \randtt, \yacht\ and \seeds\ respectively.

In the second transformation, the number of near-duplicates we generate for each data point follows the \emph{power-law} distribution. More precisely, we randomly order the points as $\bx_1, \bx_2, \ldots, \bx_n$, and for each point $\bx_i$, we add $\lceil n \cdot i^{-1} \rceil$ noisy points in the same way as above.
We denote the resulting datasets as \randfivepl, \randttpl, \yachtpl\ and \seedspl\ respectively. 



\paragraph{Method \& Measurements}
For each dataset, we run each of our proposed sampling algorithms a large number of times (denoted by $\nruns$, which ranges from $200,000$ to $500,000$), and count the number of times each group being sampled. We report the following results measuring the performance of our proposed algorithms.  
\begin{itemize}
\item \pTime: Processing time per item; measured by millisecond. The running time is tested using single thread.
\item \pSpace: Peak space usage throughout the streaming process; measured by word. 
\end{itemize}
We record \pTime\ and \pSpace\ by taking the average of 100 runs where in each run we scan the whole data stream.

The following two accuracy measurements for the $\ell_0$-sampling algorithms follow from \cite{CF14}.
\begin{itemize}
\item \stdDevNm: Let $F_0$ be the number of groups, and let $f^* = \frac{1}{F_0}$ be the target probability. We calculate the standard deviation of the empirical sampling distribution and normalize it by $f^*$.
\item \maxDevNm: We calculate the normalized maximum deviation of the empirical sampling distribution as 
$$\textstyle \max_{i}\left\{\frac{|f_i - f^*|}{f^*}\right\},$$ where $f_i$ is the empirical sampling probability of the $i$-th group.
\end{itemize}

We will also visualize the number of times each group being sampled.  

For the ease of presentation, we use IW and SW to represent infinite window and sliding windows respectively.  

All of the eight datasets are randomly shuffled before being fed into our algorithms as data streams. For the IW case, we return the sample at the end of a data stream.  For the SW, we fix the window size $w=200$ or $w=1000$. The window then slides over the data stream and we get the sample at the end of the data stream. Note that this is equivalent to sampling in a random window because the dataset has been randomly shuffled.



\paragraph{Computational Environment}
Our algorithms are implemented in C++ and the visualization code is implemented in python+matplotlib. We run our experiments in a PowerEdge R730 server equipped with 2 x Intel Xeon E5-2667 v3 3.2GHz. This server has 8-core/16-thread per CPU, 192GB Memeory and 1.6TB SSD.


\subsection{Computing $\adj(p)$ in $\mathbb{R}^d$}
Before presenting the experimental results, we discuss some important details of our implementation. 

Recall the definition of $\adj(p)$ introduced in Section~\ref{sec:2D}:
$$\adj(p) = \{C \in \Grid\ |\ d(p, C) \le \alpha\}.$$
In Section~\ref{sec:2D} we did not spell out how to compute $\adj(p)$ in $\mathbb{R}^d$ because our discussion focused on the case $d = \Theta(1)$, where computing $\adj(p)$ only takes $O(1)$ time.  However, the naive implementation that we enumerate all the adjacent cells of $\cell(p)$ and test for each cell $C$ whether we have $d(p, C) \le \alpha$ takes $\Theta(d\cdot 3^d)$ time: we have $3^d$ cells to exam, and each cell has $d$ coordinates. This is expensive for large $d$. In the following we illustrate how to compute $\adj(p)$ efficiently in practice.

According to Lemma \ref{lem:small-Sr}, the expected size of $\adj(p)$ is always bounded by a small constant given a sufficiently large separation ratio. Therefore it is possible to compute $\adj(p)$ more efficiently if we can avoid the exhaustive enumeration of the adjacent cells of $\cell(p)$. We approach this by effectively pruning cells that are impossible to meet the requirement that $d(p, C) \le \alpha$.

To simplify the presentation, we set the side length of the grid $\mathbb{G}$ to be $1$ and rescale the value $\alpha$ accordingly. We further identify the grid with the Cartesian coordinates with the origin $\mathbf{0} = (0, \ldots, 0)$.   Consider a point $p = (x_1, x_2, \ldots, x_d)$. To calculate the distance from $p$ to a cell $C$ that is adjacent to $\cell(p)$, we move $p$ to the nearest point in $C$ and record the distance being moved. The movement can be done sequentially: first in the direction of $x_1$, and then in the direction of $x_2$, $\ldots$ until $x_d$.

Figure \ref{fig:nearest-points} gives an illustration of the nearest points of $p$  in $\mathbb{R}^2$. To enumerate all those nearest points, we iterate the coordinates of $p$ from $x_1$ to $x_d$. For $x_i$, we have three options: (1) move to $\lfloor x_i \rfloor$; (2) move to $\lceil x_i \rceil$; and (3) do not move. Consequently we have $3^d$ different nearest points, and thus $3^d$ different cells which are  the cells adjacent to $\cell(p)$ including $\cell(p)$ itself. 
We then perform the enumeration using a DFS search and prune the search as long as the accumulated distance exceeds $\alpha$.  The details of this procedure are presented in Algorithm \ref{alg:searchAdj} and Algorithm \ref{alg:adj}.  

\begin{figure}
  \centering
  \includegraphics[width=0.28\textwidth]{figures-new/nearest-points.pdf}
  \caption{Nearest points of $p = (x_1, x_2) \in \mathbb{R}^2$ (red point). The eight light blue cells are cells adjacent to $\cell(p)$. There are eight black points, each of which is the nearest point from $p$ in the corresponding cell} 
  \label{fig:nearest-points}
\end{figure}

\begin{algorithm}[t]
  \DontPrintSemicolon
  \tcc{$p = (x_1, \ldots, x_d) \in \mathbb{R}^d$;
    $i = 1, 2, \ldots, d$ is the depth of the DFS search;
    $s$ is the square of the distance of the movement
  }
  \If{$s > \alpha^2$}{
    \tcc{the distance of the movement exceeds $\alpha$; no need to continue the search}
    \Return\;
  }
  \If{$i > d$}{
    $q \gets (y_1, \ldots, y_d)$\;
    \tcc{Since $q$ is on the boundary, we add $0.01\cdot (q - p)$ to make sure that it moves inside a cell so that $\cell(q')$ is well defined
    }
    $q' \gets q + 0.01\cdot (q - p)$\;
    Emit $\cell(q')$\;
    \Return\;
  }
  \tcc{move $x_i$ to $\lfloor x_i \rfloor$}
  \searchAdj\parbox[t]{.6\linewidth}{
    $(p, i+1, s + (\lfloor x_i \rfloor - x_i)^2,$\\
    $(y_1,\ldots, y_{i-1}, \lfloor x_i \rfloor, \bot, \ldots) )$\;}
  \tcc{no movement}
  \searchAdj\parbox[t]{.6\linewidth}{
    $(p, i+1, s,$\\
    $(y_1,\ldots, y_{i-1},x_i, \bot, \ldots) )$\;}
  \tcc{move $x_i$ to $\lceil x_i \rceil$}
  \searchAdj\parbox[t]{.6\linewidth}{
    $(p, i+1, s + (\lceil x_i \rceil - x_i)^2,$\\
    $(y_1,\ldots, y_{i-1}, \lceil x_i \rceil, \bot, \ldots) )$\;}
\caption{\searchAdj$(p, i, s, (y_1, \ldots, y_{i-1}, \bot, \ldots, \bot))$}
\label{alg:searchAdj}
\end{algorithm}

\begin{algorithm}[t]
  \DontPrintSemicolon
  $q \gets (\bot, \bot, \ldots, \bot) \in \mathbb{R}^d$\;
  \Return all cells emitted by \searchAdj$(p, 1, 0, q)$
\caption{\adj$(p)$}
\label{alg:adj}
\end{algorithm}

\setlength{\belowcaptionskip}{-10pt}


\subsection{Results and Discussions}


We visualize our experimental results in Figure~\ref{fig:ptime}-\ref{fig:seeds-pl}. Figure \ref{fig:ptime} and Figure \ref{fig:pspace} show the results for time and space respectively, and Figure \ref{fig:deviation} presents the deviations of the empirical sampling distributions.  Figure \ref{fig:rand-5}-\ref{fig:seeds-pl} visualize the empirical sampling distribution of each dataset.



\begin{figure*}[h]
  \centering
  \includegraphics[width=0.7\textwidth]{figures-new/ptime}
  \caption{\pTime}
  \label{fig:ptime}
\end{figure*}

\begin{figure*}[h]
  \centering
  \includegraphics[width=0.7\textwidth]{figures-new/pspace}
  \caption{\pSpace}
  \label{fig:pspace}
\end{figure*}

\setlength{\belowcaptionskip}{-10pt}

\begin{figure*}[h]
  \centering
  \includegraphics[height=0.38\textwidth,width=0.8\textwidth]{figures-new/deviation}
  \caption{\maxDevNm\ and \stdDevNm}
  \label{fig:deviation}
\end{figure*}

\setlength{\belowcaptionskip}{-30pt}



\begin{figure*}[ht]
     \centering
     \subfloat[][IW, $\nruns=200,000$]{\includegraphics[height=0.15\textwidth,width=0.25\textwidth]{figures-new/d5-500}}
     \subfloat[][SW, $w=200, \nruns=200,000$]{\includegraphics[height=0.15\textwidth,width=0.25\textwidth]{figures-new/d5-500-sw}}
     \subfloat[][SW, $w=1000, \nruns=200,000$]{\includegraphics[height=0.15\textwidth,width=0.25\textwidth]{figures-new/d5-500-sw-1000}}
     \caption{\randfive\ dataset}
     \label{fig:rand-5}
\end{figure*}

\setlength{\belowcaptionskip}{-30pt}


\begin{figure*}[ht]
     \centering
     \subfloat[][IW, $\nruns=200,000$]{\includegraphics[height=0.15\textwidth,width=0.25\textwidth]{figures-new/d20-500}}
     \subfloat[][SW, $w=200,\nruns=200,000$]{\includegraphics[height=0.15\textwidth,width=0.25\textwidth]{figures-new/d20-500-sw}}
     \subfloat[][SW, $w=1000,\nruns=200,000$]{\includegraphics[height=0.15\textwidth,width=0.25\textwidth]{figures-new/d20-500-sw-1000}}
     \caption{\randtt\ dataset}
     \label{fig:randtt}
\end{figure*}

\setlength{\belowcaptionskip}{-30pt}

\begin{figure*}[ht]
     \centering
     \subfloat[][IW, $\nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/yacht-inf}}
     \subfloat[][SW, $w=200, \nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/yacht-sw}}
     \subfloat[][SW,$w=1000, \nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/yacht-sw-1000}}
     \caption{\yacht\ dataset}
     \label{fig:yacht}
\end{figure*}

\setlength{\belowcaptionskip}{-30pt}

\begin{figure*}[ht]
     \centering
     \subfloat[][IW, $\nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/seeds}}
     \subfloat[][SW, $w=200, \nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/seeds-sw}}
     \subfloat[][SW, $w=1000, \nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/seeds-sw-1000}}
     \caption{\seeds\ dataset}
     \label{fig:seeds}
\end{figure*}

\setlength{\belowcaptionskip}{-30pt}

\begin{figure*}[ht]
     \centering
     \subfloat[][IW, $\nruns=200,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/d5-500-pl}}
     \subfloat[][SW, $w=200, \nruns=200,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/d5-500-sw-pl}}
     \subfloat[][SW, $w=1000, \nruns=200,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/d5-500-sw-pl-1000}}
     \caption{\randfivepl\ dataset}
     \label{fig:rand-5-pl}
\end{figure*}

\setlength{\belowcaptionskip}{-30pt}

\begin{figure*}[ht]
     \centering
     \subfloat[][IW, $\nruns=200,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/d20-500-pl}}
     \subfloat[][SW, $w=200,\nruns=200,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/d20-500-sw-pl}}
     \subfloat[][SW, $w=1000, \nruns=200,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/d20-500-sw-pl-1000}}
     \caption{\randttpl\ dataset}
     \label{fig:randtt-pl}
\end{figure*}

\setlength{\belowcaptionskip}{-30pt}

\begin{figure*}[ht]
     \centering
     \subfloat[][IW, $\nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/yacht-inf-pl}}
     \subfloat[][SW, $w=200, \nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/yacht-sw-pl}}
     \subfloat[][SW, $w=1000, \nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/yacht-sw-pl-1000}}
     \caption{\yachtpl\ dataset}
     \label{fig:yacht-pl}
\end{figure*}


\setlength{\belowcaptionskip}{-30pt}

\begin{figure*}[ht]
     \centering
     \subfloat[][IW, $\nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/seeds-pl}}
     \subfloat[][SW, $w=200, \nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/seeds-pl-sw}}
     \subfloat[][SW, $w=1000,\nruns=500,000$]{\includegraphics[height=0.17\textwidth,width=0.25\textwidth]{figures-new/seeds-pl-sw-1000}}
     \caption{\seedspl\ dataset}
     \label{fig:seeds-pl}
\end{figure*}


We now discuss these results in words.


\paragraph{Accuracy}
From Figure~\ref{fig:rand-5}-\ref{fig:seeds-pl} (in the appendix) we can see that the empirical sampling distributions of our algorithms are very close to the uniform distribution. This can be further supported by the results presented in Figure~\ref{fig:deviation} where in all datasets, \stdDevNm\ is no larger than $0.1$ and \maxDevNm\ is no larger than $0.25$.

From Figure~\ref{fig:deviation} we observe that SW-1000 (i.e. $w = 1000$) always has larger \stdDevNm\ and \maxDevNm\ than SW-200.  This is because when the window size increases, more groups will be included in the window and consequently the frequency that each group is sampled will decrease, rendering a larger variance.
%It is also clear that the accuracy of IW is generally slightly better than SW-1000, which indicates that the IW algorithm is more stable than the SW algorithm.


\paragraph{Running Time}
The IW algorithm runs extremely fast. It can be learned from Figure~\ref{fig:ptime} that the processing time per item is only $1\sim3\times 10^{-5}$ second using single thread. The processing time per item of the SW algorithm is $7\sim 23 \times 10^{-5}$ second, which is about $4\sim 10$ times slower than that of the IW algorithm. This is mainly because the SW algorithm is much more complicated than the IW algorithm and involves a larger operation overhead ($\log w$ levels, pruning, split, merge, etc.).

By comparing the results for datasets \randfive, \randtt, \randfivepl\ and \randttpl, we observe that the running time increases when the dimension $d$ increases. This is due to the fact that manipulating vectors takes more time when $d$ increases.


\paragraph{Space Usage}
Figure~\ref{fig:pspace} demonstrates the space usage of our algorithms on different datasets. We observe that the SW algorithm consistently uses more space than the IW algorithm in all datasets. 

However, unlike the running time where a difference of $10\times$ has been observed, the SW algorithm only uses up to $1.5\times$ space of that of the IW algorithm.   One explanation for such a phenomenon is that the space analysis in the proof for Theorem~\ref{thm:SW} may be a bit loose.  The pruning step at Line~\ref{line:c-1-5}-\ref{line:c-2} may happen very frequently.  Since the sampling ratio between consecutive levels only differ by a factor of $2$, one may expect that except for the top level, the expected number of points stored in all the subsequent levels would be small.  Therefore it may be possible to prove a better space upper bound under the same successful probability guarantee.  Of course the split/merge procedures may complicate such an analysis, and we leave this as a future work.  

We comment that if we can reduce the theoretical space usage then we may reduce the theoretical processing time per item as well.  However, as mentioned above that the practical time performance also depends the complexity of the algorithm/codes, which may easily generate a constant factor overhead.


%by the following reason: we use the {\em peak} space to measure the space usage.  Algorithm~\ref{alg:SW-R} is simpler and more stable than Algorithm~\ref{alg:IW}, although in the final SW algorithm we may use up to $\log w$ instances of Algorithm~\ref{alg:SW-R}. As a result, it is unlikely for the SW algorithm to have extreme space usage.


